ScaleCall -- Agentic Tool Calling at Scale for Fintech: Challenges, Methods, and Deployment Insights

While Large Language Models (LLMs) excel at tool calling, deploying these capabilities in regulated enterprise environments such as fintech presents unique challenges due to on-premises constraints, regulatory compliance requirements, and the need to disambiguate large, functionally overlapping toolsets. In this paper, we present a comprehensive study of tool retrieval methods for enterprise environments through the development and deployment of ScaleCall, a prototype tool-calling framework within Mastercard designed for orchestrating internal APIs and automating data engineering workflows. We systematically evaluate embedding-based retrieval, prompt-based listwise ranking, and hybrid approaches, revealing that method effectiveness depends heavily on domain-specific factors rather than inherent algorithmic superiority. Through empirical investigation on enterprise-derived benchmarks, we find that embedding-based methods offer superior latency for large tool repositories, while listwise ranking provides better disambiguation for overlapping functionalities, with hybrid approaches showing promise in specific contexts. We integrate our findings into ScaleCall's flexible architecture and validate the framework through real-world deployment in Mastercard's regulated environment. Our work provides practical insights into the trade-offs between retrieval accuracy, computational efficiency, and operational requirements, contributing to the understanding of tool-calling system design for enterprise applications in regulated industries.

==> Sections/Application.tex <==
\section{Application}



==> Sections/Intro-3.tex <==
\section{Introduction}

Tool calling has emerged as a key capability of large language models (LLMs), enabling them to interpret natural language instructions and dynamically invoke both internal and external application programming interfaces (APIs) or computational functions~\cite{schick2023toolformer, yao2023react, qin2023tool, patil2023gorilla}. This expands the role of LLMs from passive information retrievers to active agents capable of orchestrating workflows, executing operations, and integrating with real-world software systems. Recent research has demonstrated the promise of tool calling in general-purpose applications such as code generation~\cite{qin2023tool}, web automation~\cite{yao2023react}, and task decomposition~\cite{schick2023toolformer}, particularly in open-domain settings involving cloud-based or public APIs.

However, deploying tool-calling agents in regulated enterprise settings, such as financial services, presents unique challenges~\cite{schuman2025ai_pilots}. These environments feature complex internal toolchains composed of hundreds of proprietary services, including microservices and externally proxied APIs. Such tools often lack standardized documentation, exhibit overlapping naming conventions, and are governed by strict access controls. Regulatory compliance further imposes constraints around data handling, auditability, and system security. These issues are magnified in on-premises deployments, where agents must operate without access to external services or cloud-native tooling.

Emerging standards such as the \textit{Model Context Protocol} (MCP)~\cite{anthropic2024mcp, modelcontextprotocol2024} aim to simplify tool integration by providing structured interfaces between LLMs and external systems. However, their practical adoption in large-scale enterprise environments remains limited. Legacy systems, jurisdiction-specific compliance requirements, and fragmented tool repositories complicate the integration of such protocols within real-world infrastructure.

Consider, for instance, a Mastercard engineer automating account aggregation via Mastercard’s Open Banking APIs~\cite{mastercard_openbanking}. This task requires coordination with internal consent management services that may expose similarly named endpoints (e.g., \texttt{getConsentDetails}) but differ in authorization logic, jurisdictional constraints, or intended business contexts. Without precise disambiguation, an LLM agent risks invoking the wrong service—leading to silent failures or policy violations. These scenarios demand domain-aware retrieval, execution gating, and permission validation—capabilities often missing from tool-calling systems designed for open or SaaS environments.

These challenges can be grouped into four key dimensions: scalability, retrieval precision, deployment constraints, and functional scope. Enterprise environments often contain hundreds of overlapping tools, making similarity-based retrieval insufficient for accurate selection. As shown in recent benchmarks such as ToolRet~\cite{shi2025retsavvy}, embedding-based approaches struggle to disambiguate between functionally similar tools without contextual reasoning. Moreover, most frameworks assume cloud-native architectures and overlook the constraints of on-premise settings, such as limited internet access, data privacy requirements, and organizational firewalls. Finally, tool-calling systems must support robust execution, including permission-aware validation, error recovery, and multi-turn reasoning—requirements that go beyond one-shot retrieval and invocation.

In this work, we focus on the problem of domain-specific tool retrieval in enterprise contexts. Our approach builds on recent progress in LLM-based reranking~\cite{sun2024chatgptgoodsearchinvestigating, shi2025retsavvy}, which demonstrate the effectiveness of prompting LLMs to perform listwise ranking of retrieval candidates. While effective in open-domain settings, these methods do not directly address the constraints and ambiguities of enterprise environments.

To bridge this gap, we propose a hybrid two-stage retrieval and reranking pipeline tailored for regulated, on-premises deployments. Our method first performs semantic retrieval to narrow down the candidate set, followed by a domain-adapted, generative listwise reranker that disambiguates between tools based on context. We evaluate this pipeline using a benchmark derived from real-world enterprise use cases, and integrate it into a modular, agent-based framework that supports the full tool-calling lifecycle.

To ensure both scalability and contextual relevance, we introduce a domain-aware evaluation strategy that combines automated syntactic checks using ChatGPT\footnote{OpenAI's ChatGPT model, a large-scale generative language model} with manual spot-checking by subject matter experts. This enables scalable yet grounded assessment of tool selection quality in realistic scenarios.

\subsection*{\textbf{Key contributions:}}

\begin{itemize}
    \item \textbf{Problem formalization for fintech:} We identify and articulate the unique challenges of deploying LLM-based tool-calling agents in regulated enterprise environments, highlighting four core dimensions: scalability, ambiguity resolution, deployment constraints, and functional scope.

    \item \textbf{Hybrid retrieval and listwise reranking:} We propose a two-stage pipeline combining embedding-based retrieval with a domain-adapted, generative listwise reranker. This enables effective disambiguation of semantically similar tools based on context.

    \item \textbf{Domain-aware evaluation framework:} We design an evaluation methodology that blends synthetic query generation, automated syntactic validation, and human-in-the-loop spot-checking to measure tool retrieval performance in enterprise settings.

    \item \textbf{Real-world validation:} We demonstrate the effectiveness of our method through internal pilot deployments in a fintech setting, offering empirical insights into practical integration, deployment, and performance.
\end{itemize}


==> Sections/Intro2.tex <==
\section{Introduction}


Tool calling has emerged as a significant capability of large language models (LLMs), enabling them to interpret natural language instructions and dynamically invoke both internal and external application programming interfaces (APIs) or computational functions \cite{schick2023toolformer, yao2023react, qin2023tool, patil2023gorilla}. This advancement expands the role of LLMs from passive information retrievers to active agents capable of orchestrating large workflows, executing operations, and integrating with existing software infrastructures. Recent research has demonstrated the potential of tool calling in general-purpose applications such as code generation \cite{qin2023tool}, web automation \cite{yao2023react}, and agent-based task delegation \cite{schick2023toolformer}, particularly when deployed in open-domain environments with public APIs or cloud-based resources.

However, the deployment of tool-calling agents in regulated enterprise settings, such as fintech, presents substantial challenges \cite{schuman2025ai_pilots}. These environments are characterized by extensive internal toolchains composed of hundreds of proprietary services, ranging from internal microservices to externally proxied APIs that frequently lack unified documentation, display semantic overlap in their naming conventions, and are governed by strict role-based access controls. Furthermore, compliance with industry regulations entails significant technical and organizational complexities. 

While emerging standards such as the \textit{Model Context Protocol} (MCP) \cite{anthropic2024mcp, modelcontextprotocol2024} aim to provide standardized interfaces for connecting AI assistants to external systems and data sources, the practical deployment of such protocols in large-scale enterprise environments remains challenging. These challenges are particularly acute within complex, security-focused infrastructures that must address information silos and legacy systems while maintaining strict compliance requirements. The integration of standardized tool-calling protocols into such environments requires careful consideration of existing enterprise architectures, security policies, and regulatory frameworks that govern data access and system interactions.

For instance, a Mastercard engineer automating account aggregation via Mastercard's Open Banking APIs \cite{mastercard_openbanking} must also interface with internal consent management services. External API specifications are typically accessible through Swagger\footnote{\url{https://swagger.io/}}, a widely-used API specification format, or developer portals. However, internal tools are often fragmented across services. These tools enforce jurisdiction-specific consent policies, retrieve masked customer identifiers, or trigger secure notifications. Despite similar interface signatures \textit{(e.g., getConsentDetails)}, these services may differ in authorization logic or usage constraints. Such differences depend on business unit or customer segment. Without precise disambiguation and strict execution gating, a tool-calling agent risks invoking the wrong service. This can result in policy violations or silent failures due to inadequate error handling. Robust deployment of tool calling in such settings requires domain-aware function selection, multi-layered permission validation, and context-grounded reasoning. These capabilities are not yet reliably supported by existing frameworks designed for open or SaaS-based environments.

These challenges are further amplified across four key dimensions when deploying tool-calling agents in fintech: scalability, retrieval logic, deployment architecture, and functional scope. Enterprise environments often involve hundreds of overlapping tools, making accurate selection difficult. As demonstrated by recent benchmarks, existing retrieval methods—typically embedding-based—struggle with disambiguation when tools have similar names or context-sensitive behavior \cite{shi2025retsavvy}. This is especially true in the absence of standardized documentation or consistent naming. 
Moreover, most tool-calling frameworks are designed for cloud-native deployments and do not account for on-premises constraints, such as strict data privacy, compliance requirements, and limited network accessibility. Their functional scope is also narrow, focusing primarily on tool retrieval  \cite{shi2025retsavvy} and invocation while overlooking broader needs like permission-aware execution, error recovery, multi-turn interaction, and domain-grounded reasoning—capabilities essential for robust and trustworthy deployment in regulated enterprise settings.


% \subsection{\textcolor{green}{Our Contribution}}\label{AA}

% To address the aforementioned limitations, we introduce a hybrid framework for enterprise-grade tool calling, designed to meet the unique requirements of internal, secure, and large-scale enterprise environments. Our approach combines embedding-based retrieval with a lightweight LLM-based reranking strategy to enable accurate and efficient tool selection, particularly in repositories with overlapping or semantically similar tool descriptions. We evaluate our framework against the ToolRet\cite{shi2025retsavvy} benchmark and demonstrate significant improvements in retrieval performance.

% Beyond isolated evaluation, we present the integration of this method within \textit{ScaleCall}, on-premises tool calling platform\mm{not sure tool or platform} tailored for fintech enterprise contexts. ScaleCall extends the hybrid selection framework with a reasoning layer for adaptive invocation, and a Natural Language Interface (NLI) that facilitates seamless interaction between the engineers and enterprise tools.  ScaleCall is designed for replicating the full toolcalling lifecycle for on-premise applications, with modular components that align with enterprise architecture, regulartory, and operational constraints. In this, We will briefly visit the application of ScaleCall which integrates with internal APIs, 
% In this work, we focus on the problem of domain-specific tool retrieval and propose a hybrid approach designed to improve tool disambiguation within enterprise settings. Our method forms a foundational component of a larger, internally developed framework that supports the full tool-calling lifecycle in regulated environments. Specifically, we propose a two-stage retrieval \& reranking mechanism that combines semantic similarity with a generative listwise reranker to distinguish between tools with overlapping functionalities. We evaluate this approach using a benchmark dataset and integrate it into a modular, agentic framework optimized for on-premises deployment. Furthermore, we develop a domain-aware evaluation strategy that combines automated syntactic checks using ChatGPT\footnote{OpenAI's ChatGPT model, a large-scale generative language model with manual spot-checking by domain experts}. This allows us to achieve both scalable and contextually grounded assessment of tool retrieval performance.\\

In this work, we address the problem of domain-specific tool retrieval in enterprise settings, where tools often exhibit overlapping functionalities and strict compliance requirements. Our approach builds upon recent advances in large language model (LLM)-based reranking \cite{shi2025retsavvy, sun2024chatgptgoodsearchinvestigating}, which demonstrate the effectiveness of LLMs as listwise rerankers in open-domain information retrieval tasks. While these methods rely on general-purpose LLMs to improve relevance ranking, they do not address challenges unique to enterprise tool retrieval—such as domain-specific ambiguity, context-sensitive usage constraints, and the need for on-premises deployment.

To bridge this gap, we propose a hybrid two-stage retrieval and reranking pipeline tailored for regulated environments. Our method first performs semantic retrieval to narrow down candidate tools, then applies a generative listwise reranker to disambiguate between candidates based on context. Unlike prior works, our reranker is domain-adapted and optimized for distinguishing tools with subtle but critical functional differences. We evaluate the system using a benchmark dataset constructed from real-world enterprise scenarios and integrate it into a modular, agentic framework that supports the full tool-calling lifecycle. To ensure both scalability and contextual reliability, we introduce a domain-aware evaluation strategy that combines automated syntactic checks using ChatGPT\footnote{OpenAI's ChatGPT model, a large-scale generative language model} with manual validation by subject matter experts. This evaluation framework allows us to systematically assess tool relevance while accounting for enterprise-specific constraints.

To summarize, our contributions are as follows:
\begin{itemize}
\item \textbf{Formalization of Enterprise Tool-Calling Challenges:} We identify and characterize the specific obstacles hindering the deployment of LLM-based tool-calling systems in regulated, on-premises enterprise environments—focusing on scalability, ambiguity resolution, infrastructural constraints, and evaluation gaps.

\item \textbf{List-wise Generative Reranking for Tool Disambiguation:} We introduce and evaluate a novel reranking stage that leverages a large language model for sophisticated, context-aware ranking. By prompting the LLM to perform a listwise, comparative judgment over the top candidates, our method moves beyond simple similarity scores to effectively disambiguate functionally overlapping tools.

% \item \textbf{Modular Agentic Framework for On-Prem Deployment:} We integrate the proposed retrieval method into a modular, agent-based system (ScaleCall) designed for secure, on-premises environments. The framework supports full-lifecycle orchestration, including permission validation, tool invocation, and conversational interaction.

\item \textbf{Multi-Layered Evaluation Strategy:} We utilise an evaluation methodology combining synthetic query generation via LLMs and expert-curated validation, enabling scalable yet domain-aligned benchmarking of tool retrieval quality.

\item \textbf{Real-World Validation and Insights:} We report empirical results from internal pilot deployments in a fintech setting, demonstrating the practical utility of our approach and distilling lessons for enterprise-grade tool-calling systems.
\end{itemize}











% Through this work, we aim to bridge the gap between academic exploration and enterprise application of tool calling, offering a blueprint for secure, efficient, and intelligent tool-enabled LLM systems within organizational boundaries.


  



 









% To address this bottleneck, the most dominant approach has been to use Retrieval Augmented Generation (\mm{RAG, please add a ref}). This method aims to dynamically retrieve the relevant tools based on query similarity. 

% while still relevant, the retrieved tools can lead to prompt bloat which consumes a large portion of the context window. Finally, this approach is vulnerable to retrieval errors if tools are semantically similar but functionally incorrect







==> Sections/Related.tex <==
\section{Related Work}

Research on tool-calling has gained significant momentum in recent years \cite{qin2023toolllmfacdd, patil2023gorilla, yao2023reactsyting}; however, most practical implementations are optimized for cloud-based, open-domain environments and fall short of meeting the requirements of regulated sectors such as finance and healthcare. As enterprises increasingly pursue hybrid AI systems that blend language understanding with operational execution, there is a pressing need for secure, interpretable, and scalable on-premises architectures that align with organizational constraints. This gap motivates the development of frameworks capable of navigating enterprise-specific infrastructure, access control, and tool heterogeneity. A prominent example of such a high-level orchestration framework is HuggingGPT \cite{shen2023hugginggpt}, where an LLM acts as a controller to select and coordinate specialized models. However, like many others, it is primarily designed for open, cloud-based settings. \\

Current approaches to tool calling typically follow one of two paradigms: retrieval-augmented generation (RAG) and instruction-following LLMs with in-context execution capabilities \cite{shi2025retsavvy, patil2023gorilla}. RAG-based systems retrieve relevant tools based on semantic similarity and condition the LLM with their descriptions to generate function calls, whereas instruction-tuned models embed the tool context within prompts and rely on the model to perform reasoning and execution. Although these paradigms have shown promise in general settings, they often assume standardized tool documentation, cloud-native APIs, and unconstrained token budgets—assumptions that rarely hold in enterprise-scale systems. \\

The task of tool calling can be further decomposed into two stages: tool retrieval and tool execution. The retrieval phase involves selecting the most appropriate tool (e.g., API or internal function) for a given query. Foundational methods employ embedding-based similarity search over tool descriptions \cite{qin2023toolllmfacdd}, as seen in frameworks like LangChain and OpenAI’s function calling interface. To address retrieval ambiguity, several recent works introduce more sophisticated mechanisms. ToolLLM, for instance, employs LLM-based entailment reranking, while RETSavvy uses contrastive learning to disambiguate semantically similar tools \cite{shi2025retsavvy}. Another approach focuses on improving the query itself; for instance, Kachuee et al. \cite{kachuee2024improving} use an LLM to reformulate user queries to be more effective for embedding-based search. Despite these advances, tool retrieval remains challenging in enterprise environments where tool repositories often include hundreds of overlapping functions, minimal documentation, and domain-specific naming conventions. \\

To address retrieval ambiguity, several recent works introduce more sophisticated reranking mechanisms. The most common are pointwise cross-encoders, which score each (query, tool) pair in isolation. The ToolRet benchmark reports strong results using this method [6]. A more recent paradigm involves using general-purpose LLMs as the reranker. This is often accomplished with structured frameworks like RankGPT, which may use permutation or sliding-window algorithms to manage long candidate lists \cite{sun2024chatgptgoodsearchinvestigating}. Our work is more closely aligned with an emerging trend of direct, single-pass listwise reranking, as explored by Zhang et al. \cite{zhang2023rankwithoutgpt}. We contribute to this paradigm by proposing a direct, single-pass listwise prompting strategy, designed to be a simple, reproducible, and powerful method for leveraging an LLM's full contextual reasoning over a candidate set.

Once a tool is selected, the execution phase involves generating structured arguments, performing the function call, and integrating outputs into the LLM’s reasoning chain. Approaches like ReAct \cite{yao2023reactsyting} use iterative action-observation loops, while Gorilla \cite{patil2023gorilla} and ToolLLM enhance execution precision through schema modeling and supervised fine-tuning. However, these systems often neglect the operational realities of enterprise usage—such as the need for secure sandboxing, permission validation, and robust error handling. Moreover, as highlighted by RETSavvy \cite{shi2025retsavvy}, even state-of-the-art LLM-based retrievers fail to consistently select the correct tool when presented with abstract or ambiguous task descriptions. This underscores a persistent performance gap and highlights the importance of domain-specific reasoning, layered retrieval strategies, and feedback mechanisms—elements our proposed framework is designed to address. \\

==> Sections/data_evaluation_strategy.tex <==
\section{Data and Evaluation Strategy}


% As part of this work, we are developing both a tool retrieval strategy and an integration framework tailored to internal enterprise use cases. Our approaches for tool retrieval are evaluated using the publicly available ToolRet benchmark\footnote{\url{https://huggingface.co/mangopy/ToolRet-trained-e5-base-v2}, accessed June 2025} to ensure the generalizability and validity of our results. Evaluation follows the standard metrics recommended by the benchmark authors. 

% % In parallel, our internal framework, \textit{ScaleCall}, is designed to integrate with enterprise APIs and adheres to a customized evaluation strategy that complies with the organization’s data-siloing and security policies.



% \subsection{Benchmark Dataset and Evaluation Metrics: ToolRet}\label{toolret_metrics}

% We evaluate our retrieval approaches using ToolRet\cite{shi2025retsavvy}, a large-scale benchmark specifically designed for tool retrieval in LLM-based systems. As summarized in Table\ref{tab:toolret_summary} (first column), the dataset comprises 7,615 retrieval tasks constructed over a corpus of more than 43,000 tools, aggregated from over 30 sources including web APIs, software functions, and user-defined tools. Each task includes a natural language query and corresponding instruction, along with tool metadata—such as name and description—and an annotated ground-truth tool ID for evaluation. A representative example is provided in Table~\ref{tab:toolret_example}.



% \begin{table*}[th]
% \centering
% \scriptsize
% \setlength\tabcolsep{4pt}
% \caption{ToolRet Dataset Statistics: Comparison between reported and observed values. The reported statistics are taken from the original release paper (ToolRet\cite{shi2025retsavvy}), while the observed statistics are derived from our own analysis of the benchmark, accessed via the Hugging Face GitHub repository\footnote{\url{https://huggingface.co/datasets/mangopy/ToolRet-Queries/tree/main}} on July 7, 2025. The "Source Datasets" count could not be verified as the provided data was pre-processed and aggregated, hence it is marked as (–) in our analysis.}

% \begin{tabular}{p{5.2cm} p{2.4cm} p{2.8cm}}
% \toprule
% \textbf{Statistic} & \textbf{As Reported} & \textbf{Observed} \\
% \midrule

% \rowcolor{blue!5}
% Tool Corpus Size & 43,000+ & 44453 \\
% \rowcolor{blue!5}
% Source Datasets & 30+ & -- \\

% \# Retrieval Tasks & 7,615 & 7,961\\
% \quad -- Web API Retrieval Tasks & 4,916 & 5,230\\
% \quad -- Code Function Retrieval Tasks & 950 & 1,749\\
% \quad -- Customized App Retrieval Tasks & 1,749 & 982 \\
% \addlinespace
% \# Tools & 43,215 & 44,453 \\
% \quad -- Web APIs & 36,978 & 37,292 \\
% \quad -- Code Functions & 3,794 & 3,794 \\
% \quad -- Customized Apps & 2,443 & 3,367 \\

% % \rowcolor{blue!5} Annotations & Query, Instruction, Description, Tool ID & Same \\

% \addlinespace
% Avg. Query / Instruction Length (tokens) & 46.87 / 43.43 & 34.98 / 35.67 \\
% Avg. Tool Documentation Length (tokens) & 174.56 & 68.0\\
% \bottomrule
% \end{tabular}
% \label{tab:toolret_summary}
% \end{table*}



% \begin{table*}[ht]
% \centering
% \scriptsize
% \caption{Sample entry from the TOOLRET benchmark dataset. For our use case, the attributes of interest are \texttt{Query}, \texttt{Instruction}, \texttt{Tool ID}, and \texttt{Description}. The \texttt{Tool Name} field is used solely for tool mapping during retrieval.}
% \begin{tabular}{p{3cm} p{10cm}}
% \toprule
% \textbf{Attribute} & \textbf{Example Value} \\
% \midrule
% Query & \makecell[{{p{10cm}}}]{How can I resize an image to specific dimensions?} \\
% Instruction & \makecell[{{p{10cm}}}]{Use a tool that resizes an image to the specified width and height while maintaining the aspect ratio.} \\
% Tool Name & \makecell[{{p{10cm}}}]{\texttt{resize\_image\_tool}} \\
% Description & \makecell[{{p{10cm}}}]{Resizes a given image to the specified width and height. Maintains aspect ratio by default. Accepts input as an image URL or base64 string, and returns the resized image in base64 format.} \\
% Category & \makecell[{{p{10cm}}}]{Web API} \\
% Tool ID & \makecell[{{p{10cm}}}]{\texttt{tool\_4398}} \\
% Domain & \makecell[{{p{10cm}}}]{Image Processing} \\
% Input Schema & \makecell[{{p{10cm}}}]{\{ "image": "string", "width": "int", "height": "int" \}} \\
% Output Schema & \makecell[{{p{10cm}}}]{\{ "resized\_image": "string" \}} \\
% \bottomrule
% \end{tabular}
% \label{tab:toolret_example}
% \end{table*}

% we observed minor deviations in the total counts of tasks and tools compared to the statistics originally reported in [6]. While the exact reason for this discrepancy is not specified in the dataset's documentation, potential causes include subsequent dataset updates or variations in data processing scripts. Our evaluation proceeds using the observed data counts, ensuring our results are grounded in the specific artifact we utilized. 

% We utilize the dataset to address the tool retrieval task, which can be formalized as follows: given a user query ($\pm$~\texttt{instruction}), the system must identify the most appropriate tool from a large candidate library. Our evaluation is conducted independently on each subset of the dataset, and the results are aggregated to provide a comprehensive assessment of overall performance.

% Following the established evaluation protocol of the ToolRet benchmark, we assess system performance using a standard suite of information retrieval metrics, namely:

% \begin{itemize}
%     \item \textit{Success Rate (P@1)}: The primary accuracy metric. It reports the percentage of queries for which the top-ranked tool returned by the system is correct.
    
%     \item \textit{Recall@k (R@k)}:The percentage of queries where the correct tool is present within the top-$k$ retrieved results. We report both $R@1$ and $R@10$.
    
%     \item \textit{Precision@k (P@k)}: The fraction of the top-$k$ retrieved tools that are relevant. We report $P@1$ and $P@10$.
    
%     \item \textit{Completeness@k (C@k)}: The percentage of queries where all ground-truth tools are found within the top-$k$ results.
    
%     \item \textit{nDCG@k (N@k)}: Normalized Discounted Cumulative Gain, which evaluates the ranking quality by assigning higher scores to correct tools ranked earlier.
% \end{itemize}


==> Sections/draft.tex <==
\section{Draft}


\subsection{Background \& Motivation}\label{AA}

The rapid evolution of large language models (LLMs) has introduced new possibilities for enterprise automation and human-computer interaction. One of the most transformative capabilities enabled by LLMs is tool calling \mm{ref} —the ability to interpret user intent and dynamically identify, select, and invoke APIs or computational services based on natural language instructions. This functionality positions LLMs not merely as conversational agents, but as intelligent orchestrators capable of executing tasks, interfacing with complex software ecosystems, and enabling dynamic service integration.


Such capabilities align closely with enterprise demands for scalable automation, intelligent task delegation, and adaptive system integration. However, deploying LLM-based tool calling frameworks in enterprise environments presents a distinct set of challenges. Unlike public, cloud-based applications, enterprise settings are governed by restricted data privacy and compliance requirements, necessitating on-premises deployment. Additionally, these environments often rely on heterogeneous and legacy tool ecosystems, as well as proprietary internal APIs that require robust and explainable integration mechanisms.

Research on tool-calling has gained significant momentum \mm{ref, ref}; however, most practical implementations are designed for open, cloud-based environments and often fall short of meeting the requirements of regulated industries such as fintech. As enterprises increasingly pursue hybrid AI systems that integrate language-based reasoning with operational execution, there is a pressing need for on-prem tool-calling architectures that are secure, interpretable, and scalable—capable of functioning within the constraints of complex enterprise infrastructures.




\subsection{The Current Approaches}\label{AA}
Recent research has explored tool calling from various angles, primarily focusing on cloud-native, general-purpose settings \mm{ref}. Approaches can be broadly categorized into retrieval-augmented generation (RAG) frameworks \mm{ref} and instruction-tuned LLMs with in-context tool execution \mm{ref}. The RAG paradigm involves retrieving candidate tools based on semantic similarity and prompting the LLM to generate the appropriate call. The LLM-based approach applies carefly crafted prompts aligned with the tool context in order to retireve and execute the tool. 

In terms of the extend, the work in tool calling can be decomposed into two distinct stages:

\paragraph{\textbf{tool retrieval} }
This task is defined as the process of selecting the most appropriate API or function in response to a user query. It is the foundational to any tool-calling system in large language models (LLMs). Early and widely adopted methods leverage semantic similarity, where both the user query and tool descriptions (e.g., function names, docstrings, or metadata) are embedded into a shared vector space. The retrieval is then performed using embedding-based similarities.This approach, used in frameworks such as LangChain\footnote{\url{https://python.langchain.com/docs/how_to/function_calling/}}.
 and OpenAI Function Calling\footnote{\url{https://platform.openai.com/docs/guides/function-calling?api-mode=chat}}. These approaches are notable for the fallback of disambiguation—particularly when tools share similar functionality or when user intent is context-dependent. Several studies have attempted to address these limitations. For instance, ToolLLM\cite{qin2023toolllmfacdd} introduces a multi-step reasoning pipeline that reranks retrieved tools using LLM-based entailment scoring. RETSavvy \cite{shi2025retsavvy} proposes contrastive learning on tool representations to better separate semantically similar tools. The work introduced through Gorilla \cite{patil2023gorilla} fine-tunes models on tool-use demonstrations to improve tool grounding. Despite these advances, tool retrieval remains challenging at enterprise scale, where repositories include hundreds of functionally similar, internally-named tools, and where token efficiency, disambiguation, and alignment with proprietary usage contexts are critical.

\paragraph{\textbf{tool execution} }
After retrieving the appropriate tool, the execution phase involves generating structured arguments, invoking the function or API, and integrating the output into the interaction. Approaches like ReAct \cite{yao2023reactsyting} use iterative reasoning-action loops to manage tool use, while ToolLLM \cite{qin2023toolllmfacdd} enhances this by modeling tool schemas for precise argument generation. Fine-tuned models like Gorilla \cite{patil2023gorilla} improve execution accuracy by learning from tool usage traces.

% The application of these still at the research level, execution in enterprise settings will likely  demands validation, error handling, and secure sandboxing, making this step a critical component in deploying reliable and compliant tool-calling systems.



 


tool selection has consistently been identified as a critical component for the effectiveness of tool-augmented AI systems and even even state-of-the-art retrieval-augmented models frequently struggle with accurately selecting the appropriate tool—particularly in cases where tool functionalities or descriptions are semantically similar \cite{shi2025retsavvy}. This limitation poses a significant challenge for systems that rely on precise tool invocation to complete tasks reliably.




A notable example in tool selection is  the work by \cite{shi2025retsavvy} which takes a systematic approach to evaluate the ability of large language models (LLMs) to retrieve appropriate tools for given tasks. The work introduces a benchmark to evaluate tool selection in RAG-based systems which is used in this paper. . The authors analyze several retrieval and reranking pipelines using LLMs to perform tool matching. While this work highlights the importance of structured tool repositories and contextual reasoning, it is largely evaluated in synthetic or open-domain settings and does not address the specific demands of enterprise-grade deployments.


 The core task is to select the most suitable tool(s) for the task, without actually executing the tool—focusing purely on retrieval. The authors test both standard retrieval models and LLM-based retrievers (like LlamaIndex and RAG setups), and they compare retrieval accuracy using multiple prompting techniques (e.g., few-shot, chain-of-thought). Notably, they find that even LLMs fine-tuned on tool use do not consistently retrieve the correct tool, particularly when faced with abstract task descriptions or subtle differences in tool functionality. This suggests that current retrieval strategies fall short in tool-specific reasoning and understanding.



The results highlight a significant gap between LLMs' perceived reasoning abilities and their actual performance in practical tool retrieval







% This speedy transformation has grown the capabilities of LLMs allowing them to now query databases (\mm{Add a ref.}), execute code(\mm{, add a ref}) and interact with different software systems changing their role to intelligent agents who can perform real-world tasks (\mm{add a ref}). A place where we can especially recognize the paradigm shift is within a high stake environment such as financial technology as the ability to use natural language to bring about tangible action can prove to be crucial when automating complex workflows and improve operational efficiency (\mm{This setence seems a bit robotic. It needs a rephrase and rewriting. }).



% \subsection{\textcolor{green}{Limitations of Current Approaches}}\label{AA}

% While recent tool calling frameworks demonstrate significant potential, they face notable limitations when scaled and applied to enterprise contexts. These limitations can be broadly categorized into four dimensions: scalability, retrieval logic, deployment setting, and functional scope.

% From a scalability perspective, the transition from small-scale prototypes to enterprise-grade systems introduces substantial performance constraints. In realistic enterprise scenarios, systems must support the selection and invocation of hundreds or even thousands of tools, many of which exhibit overlapping descriptions and interface signatures \mm{add appropriate references for scale and thresholds}. This challenge directly relates to the second limitation concerning retrieval and implementation logic. Predominantly, tool selection relies on semantic embedding-based retrieval, which has been shown to struggle with disambiguating tools with overlapping or context-sensitive functionalities—a common scenario in large, heterogeneous organizational environments \mm{add reference}.

% Third, in terms of deployment setting, many existing solutions are architected for cloud-native infrastructures and overlook the constraints of on-premises deployment \mm{ref}. As a result, these systems often fail to meet the stringent data privacy, security, and compliance requirements that are foundational to enterprise operations.

% Lastly, regarding functional scope, much of the existing research centers on  tool retrieval \cite{shi2025retsavvy} and invocation \mm{ref}, without addressing the broader tool calling lifecycle \mm{ref}. Enterprise applications demand systems that incorporate adaptive reasoning strategies, handle multi-turn interactions, and integrate with a natural language interface (NLI) to support end-to-end task orchestration. The absence of these capabilities constrains the utility of current frameworks in dynamic, real-world settings where contextual reasoning and user interactivity are essential.





% Additionally, the tight coupling between retrieval and generation in these models often leads to brittle behavior when faced with domain shifts or evolving tool repositories, which are commonplace in enterprise settings.


% third, while LLM-based reranking can improve selection accuracy, it introduces additional latency and computational overhead—factors that may hinder scalability and responsiveness in production-grade systems without careful optimization \mm{ref}. Most significantly, many existing solutions are designed for cloud-native deployment and lack support for on-premises integration, rendering them unsuitable for enterprises operating under strict data privacy, security, and regulatory constraints.


% Although the scale issue is apparent, we must understand that the main issue lies in how we deal with this problem. The naive approach of placing all the tool definitions in the prompt for the LLM is not applicable due to the limits on context window, token costs, and latency in inference 
